Non-Linear Coordination Graphs

Value decomposition multi-agent reinforcement learning methods learn the global value function as a mixing of each agent's individual utility functions. Coordination graphs (CGs) represent a higher-order decomposition by incorporating pairwise payoff functions and thus is supposed to have a more powerful representational capacity. However, CGs decompose the global value function linearly over local value functions, severely limiting the complexity of the value function class that can be represented. In this paper, we propose the first non-linear coordination graph by extending CG value decomposition beyond the linear case. One major challenge is to conduct greedy action selections in this new function class to which commonly adopted DCOP algorithms are no longer applicable. We study how to solve this problem when mixing networks with LeakyReLU activation are used. An enumeration method with a global optimality guarantee is proposed and motivates an efficient iterative optimization method with a local optimality guarantee. We find that our method can achieve superior performance on challenging multi-agent coordination tasks like MACO.

==> alg/dcg-greedy.tex <==
\begin{algorithm*}[h]
	\begin{algorithmic}
	\Function{greedy}{$\ve f^\text{V} \in \R^{|\Set V| \times A}, 
					\ve f^\text{E} \in \R^{|\Set E| \times A \times A},
					\Set V, \Set E, \{\Set A^i\}_{i=1}^{|\Set V|}, k
					$}
			\Comment{$A := |\cup_i \Set A^i|$}
		\State $\ve\mu^0, \bar{\ve\mu}^0 := \ve 0 \;\in\; \R^{|\Set E| \times A}$
			\Comment{messages forward ($\ve \mu$) 
					 and backward ($\bar{\ve \mu}$)}
		\State $\ve q^0 := \frac{1}{|\Set V|} \ve f^\text{V}$
			\Comment{initialize ``Q-value'' without messages}
		\State $q_\text{max} := -\infty; \quad 
				  \ve a_\text{max} := \big[\argmax\limits_{a \in \Set A^i} q^0_{ai} 
				  							  \,\big	|\, i \in \Set V \big]$
			\Comment{initialize best found solution}
		\For{ $t \;\in\; \{1, \ldots, k\}$ }  
				\Comment{loop with $k$ message passes}
			
			\For{ $e = (i,j) \;\in\; \Set E$ }
				\Comment{update forward and backward messages}
				\State $\ve \mu_e^{t} := \max\limits_{a \in \Set A^i} 
						\big\{ (q_{ia}^{t-1} \!- \bar{\mu}_{ea}^{t-1}) 
						+ \frac{1}{|\Set E|} \ve f^\text{E}_{ea} \big\}$
					\Comment{forward: maximize sender}
				\State $\bar{\ve \mu}_e^{t} := \max\limits_{a \in \Set A^j} 
						\big\{ (q_{ja}^{t-1} \!- {\mu}_{ea}^{t-1}) 
						+ \frac{1}{|\Set E|} (\ve f^\text{E}_{e})^{\!\top}_{a} \big\}$
					\Comment{backward: maximizes receiver}
				\If{ \texttt{message\_normalization} }
					\Comment{to ensure converging messages}
					
					\State $\ve \mu^{t}_e \leftarrow \ve \mu^{t}_e 
							- \frac{1}{|\Set A^j|} \sum\limits_{a \in \Set A^j} 
								\mu^t_{ea}$
						\Comment{normalize forward message}
					\State $\bar{\ve \mu}^{t}_e \leftarrow \bar{\ve \mu}^{t}_e 
							- \frac{1}{|\Set A^i|} \sum\limits_{a \in \Set A^i} 
								\bar\mu^t_{ea}$
						\Comment{normalize backward message}
				\EndIf
			\EndFor
			\For{$i \;\in\; \Set V$}
				\Comment{update ``Q-value'' with messages}
				\State $\ve q_i^t := \frac{1}{|\Set V|} \ve f^\text{V}_i 
						\;+\; \hspace{-4mm} 
							{\displaystyle\sum_{e = (\cdot,i) \in \Set E}} 
							\hspace{-3mm} \ve\mu^t_e
						\;+\; \hspace{-4mm}
							{\displaystyle\sum_{e = (i,\cdot) \in \Set E}} 
							\hspace{-3mm} \bar{\ve\mu}^t_e$
					\Comment{utility plus incoming messages}
				\State $a^t_i := \argmax\limits_{a \in \Set A^i} \{ q^t_{ia} \}$
					\Comment{select greedy action of agent $i$}
			\EndFor
			\State $q' \leftarrow \text{\sc qvalue}(\ve f^\text{V}, 
					\ve f^\text{E}, \ve a^t, \varnothing)$
					\Comment{get true Q-value of greedy actions}
			
			\If{$q' > q_\text{max}$}
				$\{ \ve a_\text{max} \leftarrow \ve a^t; \;\; 
						q_\text{max} \leftarrow q'\}$
					\Comment{remember only the best actions}
			\EndIf
		
		\EndFor
		\Return \;$\ve a_\text{max} \in \Set A^1 \times \ldots \times \Set A^{|\Set V|}$ 
			\Comment{return actions that maximize the joint Q-value}
	\EndFunction
	\end{algorithmic}
	\caption{\label{alg:greedy}
		Greedy action selection with $k$ message passes in a coordination graph.} 
\end{algorithm*}


==> alg/dec-qmix.tex <==
\begin{algorithm}[h]
\caption{DEC-QMIX\\/*Decompose QMIX function into pieces of linear functions.*/} 
\label{alg:piecewise}
\begin{algorithmic}
	\STATE {\bfseries Input:} $\mathbf{W_0}, \ve b_0, \ve W_1, b_1$ 
	
		\COMMENT {input $Q_{tot}$  parameters}
		
	\FOR{ $\ve c_p \;\in\; \{\alpha,1\}^m$}
	    \STATE  \COMMENT {($O(2^m)$}
	    
	    \STATE $\ve W_{\rho_p} = (\ve c \circ \ve W_1) \mathbf{W_0}$
	    
	    \STATE $b_{\rho_p} = (\ve c \circ \ve W_1) \ve b_0 + b1$
	
	\ENDFOR
	    
	\STATE	\RETURN each $\rho_p$ 
		\COMMENT{return}

\end{algorithmic}
\end{algorithm}

==> alg/heu-tree.tex <==
\begin{algorithm}[H]
\caption{Heuristic Action Selection Algorithm}
\begin{algorithmic}[1]
    
    \STATE Compute the weight of the mixing network and Initialize an emtpy graph
    
    \FOR {iter$=1,\cdots, n - 1$}
    
        \STATE add $e=\mathop{\arg\max}_{e \in \mathcal{E}, E \cup \{e\} \text{~is~acyclic}} f (E \cup \{e\})$ to the graph
    
    \ENDFOR
    
    \STATE Initialize the state of the activating function
    
    \FOR {iter$=1,\cdots, T$}
    
        \STATE Compute best action according to the exact value
        
        \STATE Get the state of activating function according to current actions
    
    \ENDFOR
    
    \STATE Compute best actions according to the exact value
			
\end{algorithmic}
\end{algorithm}


==> alg/hier-greedy.tex <==
\begin{algorithm*}[h]
	\begin{algorithmic}
	\Function{hier-greedy}{
        $\ve f^\text{V} \in \R^{|\Set V| \times A}, 
		\ve f^\text{E} \in \R^{|\Set E| \times A \times A},
		%[\ve W_{\Set V},\ve W_{\Set E}] \in \R^{(|\Set V|+|\Set E|) \times m},
		\mat W_0,
		\ve b_0,
		\ve W_1,
		\Set V, 
		\Set E,
		\{\Set A^i\}_{i=1}^{|\Set V|}, 
		k
		$}\\
		\Comment{$A := |\cup_i \Set A^i|$}
		
		\State $\ve h^0 := \ve 0 \;\in\; \R^{m \times |\Set V| \times A}$
		    \Comment{initialize level-1 f2v messages}
		
		\State $\ve \mu^0 := \ve 0 \;\in\; \R^{m \times |\Set V| \times A}$
		    \Comment{initialize level-1 v2f messages}
					 
		\State $\ve q^0 := \ve f^\text{V} \;\in\; \R^{|\Set V| \times A}$
			\Comment{initialize level-1 ``Q-value'' without messages}

		\State $q_\text{max} := -\infty; \ve a_\text{max} := \big[\argmax\limits_{a \in \Set A^i} q^0_{ia} \,\big	|\, i \in \Set V \big]$
			\Comment{initialize best found solution}
		
		\For{ $t \;\in\; \{1, \ldots, k\}$ }  
				\Comment{loop with $k$ message passes}

			\For{ $l \;\in\; \{1, \ldots, m\}$ }

				\State $\ve \mu_{l,\cdot,\cdot}^{t-1} := \ve q^{t-1} - \ve h_{l,\cdot,\cdot}^{t-1}$
				    \Comment{update level-1 v2f messages}
				
				\State $\cdot, \cdot, \ve h_{l,\cdot,\cdot}^{t} := \text{\sc piece-greedy}(\ve \mu_{l,\cdot,\cdot}^{t-1}, \ve f^\text{E}, \mat W_{0l}, \ve b_{l})$
				    \Comment{using level-2 message passing}
				
				\State $\ve h_{l,\cdot,\cdot}^{t} := \text{LeakyRelu}(\ve h_{l,\cdot,\cdot}^{t}) * \ve W_{1l}$
					\Comment{update level-1 f2v messages}
				
				
				\EndFor
			
			\If{ \texttt{message\_normalization} }
				
				\State $\ve h^{t}_{\cdot,\cdot} \leftarrow \ve h^{t}_{\cdot,\cdot} 
						- \frac{1}{|\Set A^j|} \sum\limits_{a \in \Set A^j} 
							h^t_{\cdot,\cdot, a}$
					\Comment{level-1 normalize message}
			\EndIf
		
			
			\For{$i \;\in\; \Set V$}
				\Comment{update ``Q-value'' with messages}
				\State $\ve q_i^t := \ve f^\text{V}_i + {\displaystyle\sum_{m \in \{1, \ldots, n\}}} \ve h^t_{m,i}$
					\Comment{utility plus incoming messages}
				\State $a^t_i := \argmax\limits_{a \in \Set A^i} \{ q^t_{ia} \}$
					\Comment{select greedy action of agent $i$}
			\EndFor
			

			\State $q' \leftarrow \text{\sc QMIX-VALUE}(\ve a^t)$
			\If{$q' > q_\text{max}$}
				$\{ \ve a_\text{max} \leftarrow \ve a^t; \;\; 
						q_\text{max} \leftarrow q'\}$
					\Comment{remember only the best actions}
			\EndIf
		
		\EndFor
		\Return \;$q_\text{max}, \ve a_\text{max} \in \Set A^1 \times \ldots \times \Set A^{|\Set V|}$ 
			\Comment{return actions that maximize the joint Q-value}
	\EndFunction
	\end{algorithmic}
	\caption{\label{alg:hier-greedy}
		Hierarchical greedy action selection from QMIX network in a coordination graph.} 
\end{algorithm*}

